Risk-aware linear bandits with convex loss

In decision-making problems such as the multi-armed bandit, an agent learns sequentially by optimizing a certain feedback. While the mean reward criterion has been extensively studied, other measures that reflect an aversion to adverse outcomes, such as mean-variance or conditional value-at-risk (CVaR), can be of interest for critical applications (healthcare, agriculture). Algorithms have been proposed for such risk-aware measures under bandit feedback without contextual information. In this work, we study contextual bandits where such risk measures can be elicited as linear functions of the contexts through the minimization of a convex loss. A typical example that fits within this framework is the expectile measure, which is obtained as the solution of an asymmetric least-square problem. Using the method of mixtures for supermartingales, we derive confidence sequences for the estimation of such risk measures. We then propose an optimistic UCB algorithm to learn optimal risk-aware actions, with regret guarantees similar to those of generalized linear bandits. This approach requires solving a convex problem at each round of the algorithm, which we can relax by allowing only approximated solution obtained by online gradient descent, at the cost of slightly higher regret. We conclude by evaluating the resulting algorithms on numerical experiments.

==> convex_risk_ts.tex <==
\section{Thompson Sampling with convex risk}

The idea of linear Thompson sampling (LinTS) is to replace the deterministic optimistic policy with a randomized exploration scheme. In what follows, we adopt the point of view of \citet{abeille2017linear} and note that their LinTS algorithm can be transposed readily in the convex risk framework (they already showed that the extension to generalized linear bandits, which is formally similar, was straightforward). 

Intuitively, the exploration process should balance \textit{concentration}, in order to remain close to the empirical risk minimizer $\wh{\theta}$ (exploitation), and \textit{anti-concentration}, to ensure sufficient exploration. This is summarized in the next definition.

\begin{restatable}[LinTS assumption]{assumption}{assumptionsiz}\label{ass:6}
	Assume we know a distribution $\cD^{\text{TS}}$ s.t a random variable $\xi\sim\cD^{\text{TS}}$ satisfies:
	\begin{enumerate}[(i)]
		\item Concentration: $\exists c, c'\in\R, \forall \delta\in(0, 1),\ \bP\left( \lVert \xi \rVert_2 \leq \sqrt{cd\log(\frac{c'd}{\delta})} \right) \geq 1 - \delta$.
		\item Anti-concentration: $\exists p>0, \forall u\in \R^d,\  \bP\left( u^\top \xi \geq \lVert u\rVert_2\right) \geq p$.
	\end{enumerate}
	
	Furthermore, for $\delta\in(0, 1)$ and $t\in\N$, we let $c^{\text{TS}}_{t}(\delta) = c^{\delta}_t \sqrt{cd\log\frac{c'd}{\delta}}$ where $c^\delta_t$ is the same as in Theorem~\ref{thm:regret_ucb}.
\end{restatable}


\begin{algorithm}[]
	\caption{LinTS for convex risk \label{algo::UCB_convex_risk}}
	\SetKwInput{KwData}{Input} 
	\KwData{horizon $T$, loss function $\cL$, regularisation parameter $\alpha$, projection $\Pi$, exploration bonus sequence $(\gamma_t)_{t\in\N}$, distribution $\cD^{\text{TS}}$.}
	\SetKwInput{KwResult}{Initialization}
	\SetKwComment{Comment}{$\triangleright$\ }{}
	\SetKwComment{Titleblock}{// }{}
	\KwResult{Observe $\cX_1$.} 
	\For{$t=1, \dots, T$}{
		$\widehat{\theta}_t \in \arg\min_{\R^d} \sum_{s=1}^{t-1} \cL(Y_s, \langle \theta, X_s\rangle) + \frac{\alpha}{2}\lVert \theta \rVert^2_2$ \Comment*[r]{Empirical risk minimization}
		$\bar{\theta}_t = \Pi(\wh{\theta}_t)$ \Comment*[r]{Project onto $\Theta$}$
		\wt{\theta}_t = \bar{\theta}_t + c^{\frac{\delta}{4T}}_t H^{\kappa \alpha}_t(\bar{\theta}_t)^{-\frac{1}{2}} \xi_t$ where $\xi_t\sim\cD^{\text{TS}}$ \Comment*[r]{Randomization}
%		\wt{\theta}_t = \bar{\theta}_t + c^{\frac{\delta}{4T}}_t (V^{\frac{\kappa \alpha}{m}}_t)^{-\frac{1}{2}} \xi_t$ \Comment*[r]{Randomization}
		$X_t = \arg\max_{x\in\cX_t} \langle\wt{\theta}_t, x\rangle$ \Comment*[r]{Play arm}
		Observe $Y_t$ and $\cX_{t+1}$.
	}
\end{algorithm}

%\begin{algorithm}[H]
%\SetAlgoLined
%\TitleOfAlgo{Exact-$\psi$-TS}
%\textbf{Input}: horizon $T$, sequence of confidence scale $(\alpha_t)_{t\leq T}$, distribution $\cD^{\text{TS}}$, regularisation parameters $\lambda$ and $\mu$.\\
%\textbf{Initialisation}: $V_1 = \mu I_d$.\\
%\For{$t=1, \dots, T$}{
%    $\widehat{\theta}_t \in \arg\min_{\theta\in\R^d} \sum_{s=1}^{t-1} \psi(Y_s - X_s^\top \theta) + \frac{\lambda}{2}\lVert \theta \rVert^2_2$,\\
%    $\tilde{\theta}_t = \wh{\theta}_t + \alpha_t V_t^{-\frac{1}{2}}\xi_t$,\\
%    Sample $\xi_t\sim \cD_\text{TS}$,\\
%    $A_t = \arg\max_{k\in[K]} X_{t, k}^\top\wt{\theta}_t$,\\
%    Observe $Y_t = Y_{t, A_t}$, $X_t = X_{t, A_t}$, $V_{t+1} = V_{t} + X_t X_t^\top$.
%}
%\end{algorithm}

\paragraph{Regret analysis}

%\begin{theorem}[Regret of $\psi$-TS]\ \\
%Let $\delta>0$, $\lambda\geq \max(1, L^2)$, $\mu \leq \frac{\lambda}{\kappa}$ the pseudo-regret of $\psi$-TS is bounded with probability at least $1-\delta$ by:
%\[R_T \leq \alpha_T(\delta/4)\Bigg[ \frac{\sqrt{cd\log(4c'dT/\delta)}}{p}\bigg( \sqrt{2Td\log(1+\frac{TL^2}{d\lambda})} + \sqrt{\frac{8T}{\lambda}\log\frac{4}{\delta}}\Bigg) + \big(\sqrt{cd\log\frac{4c'dT}{\delta}} + 1\big) \sqrt{2Td\log\bigg(1 + \frac{T L ^2}{d\lambda}\bigg)} \bigg], \]
%
%where 
%\[ \alpha_T(\delta/4) = \frac{\sqrt{\lambda}}{\kappa} \lVert \theta^* \rVert + \frac{\sigma_{\psi}}{\kappa} \sqrt{d\log\bigg(1 + \frac{T L^2}{d\lambda}\bigg) + 2\log{\frac{4}{\delta}}}.\]
%
%Keeping the dependency only on $d$ and $T$, we have with probability at least $1 - \delta$
%\[ R_T = \wt{\cO}\bigg( d^{3/2}T^{1/2}\bigg).\]
%\end{theorem}

\begin{proof}

Let $J_t(\theta) \coloneqq \max_{k\in[K]} X_{k, t}^\top \theta$, $A_t^*(\theta) \coloneqq \arg\max_{k\in[K]} X_{k, t}^\top \theta $. The pseudo regret of Thompson sampling can be decomposed as

\begin{align*}
    R_T &= \sum_{t=1}^T (X^*_t)^\top\theta^* - X_t^\top\theta^*\\
    &= \underbrace{\sum_{t=1}^T J(\theta^*) - J(\wt{\theta}_t)}_{R_T^{\text{TS, ac}}} + \underbrace{\sum_{t=1}^T \langle c_t^{\frac{\delta}{4T}}H^{\kappa \alpha}_t(\bar{\theta}_t)^{-\frac{1}{2}}\xi_t, X_t\rangle}_{R_T^{\text{TS, c}}} + \underbrace{\sum_{t=1}^T X_t^\top\bar{\theta}_t - X_t^\top\theta^*}_{R_T^{\cL}}.\\
\end{align*}

The term $R_T^{\text{TS, ac}}$ mostly depends on the exploration capacity of Thompson sampling, in particular the anti-concentration of $\cD^{\text{TS}}$, while $R_T^{\text{TS, c}}$ depends on the concentration of $\cD^{\text{TS}}$ to remain small. Finally, $R_T^{\cL}$ depends on the concentration of the projected empirical risk minimiser $\bar{\theta}$ around $\theta^*$, which derives from the construction of the projection operator $\Pi$ and Corollary~\ref{corr:conf}, but is otherwise unrelated to the properties of Thompson sampling itself. 

For a given $t\leq T$, let $R_{t, T}^{\text{TS, ac}}$, $R_{t, T}^{\text{TS, c}}$ and $R_{t, T}^{\psi}$ the one-step regrets of  $R_T^{\text{TS, ac}}$, $R_T^{\text{TS, c}}$ and $R_T^{\psi}$ respectively.

Since we are aiming at a high probability bound, it is enough to bound the regret on a high probability event. To this end, let us define
\begin{itemize}
    \item $\wh{E}_t = \{ \forall s\leq t, \lVert \wh{\theta}_s - \theta^*\rVert_{V_s} \leq \alpha_s(\delta/4) \}$,
    \item $\wt{E}_t = \{ \forall s\leq t, \lVert \wt{\theta}_s - \wh{\theta}_s\rVert_{V_s} \leq \gamma_{s, t}(\delta/4) \}$,
    \item $E_t = \wh{E}_t \cap  \wt{E}_t$.
\end{itemize}

As seen in Lemma \ref{lemma:self-normalized_bound_revisited}, $\bP\left( \wh{E}_T\right) \geq 1 - \delta/4$. Moreover,
\begin{align*}
    \bP\left( \wt{E}_T\right)  &= \bP\left( \forall t\leq T, \lVert \alpha_t(\delta/4) V_t^{-\frac{1}{2}}\xi_t\rVert_{V_t} \leq \gamma_{t, T}(\delta/4)\right) \\
    &= \bP\left( \forall t\leq T, \alpha_t(\delta/4) \lVert \xi_t\rVert_2 \leq \gamma_{t, T}(\delta/4)\right) \\
    &= \bP\left( \forall t\leq T, \lVert \xi_t\rVert_2 \leq \sqrt{cd\log\frac{c'dT}{\delta/4} }\right) \\
    &\geq 1 - \delta/4\\
\end{align*}

A simple union bound shows that $\bP\left( E_T\right)  \geq 1 - \delta/2$. Finally, $E_T\subset E_t$ for any $t\leq T$, hence $\bP\left( E_t\right)  \geq 1 - \delta/2$.
Therefore, with probability at least $1-\delta/2$, it holds that
\begin{align*} 
    R_T &= R_T\ind_{E_T}\\
    &= \sum_{t=1}^T R_{t, T}^{\text{TS, ac}}\ind_{E_T} + \sum_{t=1}^T R_{t, T}^{\text{TS, c}}\ind_{E_T} + \sum_{t=1}^T R_{t, T}^{\psi}\ind_{E_T}\\
    &\leq \sum_{t=1}^T R_{t, T}^{\text{TS, ac}}\ind_{E_t} + \sum_{t=1}^T R_{t, T}^{\text{TS, c}}\ind_{E_t} + \sum_{t=1}^T R_{t, T}^{\psi}\ind_{E_t}\\
\end{align*}

\paragraph{Bounding $R_T^{\text{TS, ac}}$}\ \\

The analysis of $R_{t, T}^{\text{TS, ac}}$ in \cite{abeille2017linear} depends only on the properties of $J$ as a support function, the anti-concentration of $\cD^{\text{TS}}$ and Azuma's concentration for supermartingales, none of which are specific to our convex regression setting. Therefore:
\[ \sum_{t=1}^T R_{t, T}^{\text{TS, ac}}\ind_{E_t} \leq \frac{\gamma_{T, T}(\delta/4)}{p}\bigg( \sqrt{2Td\log(1+\frac{TL^2}{d\lambda})} + \sqrt{\frac{8T}{\lambda}\log\frac{4}{\delta}}\bigg).\]

\paragraph{Bounding $R_T^{\text{TS, c}}$}\ \\

We have

\begin{align*}
    \lvert R_{t, T}^{\text{TS, c}}\rvert \ind_{E_t} &= \alpha_t(\delta/4) \lvert X_t^\top V_t^{-\frac{1}{2}} \xi_t\rvert \ind_{E_t}\\
    &\leq \alpha_t(\delta/4) \lVert X_t \rVert_{V_t^{-1}} \lVert \xi_t\rVert_2 \ind_{E_t}\quad \text{(Cauchy-Schwarz)}\\
    &\leq \gamma_{t, T}(\delta/4)\lVert X_t \rVert_{V_t^{-1}} \quad \text{(concentration of $\xi$ and definition of $\gamma_{t, T}(\delta/4)$)}\\
    &\leq \gamma_{T, T}(\delta/4)\lVert X_t \rVert_{V_t^{-1}}.\\
\end{align*}

Therefore :

\begin{align*}
    \sum_{t=1}^T R_{t, T}^{\text{TS, c}}\ind_{E_t} &\leq \sum_{t=1}^T \lvert R_{t, T}^{\text{TS, c}} \rvert\ind_{E_t} \\
    &\leq \gamma_{T, T}(\delta/4)\sum_{t=1}^T \lVert X_t \rVert_{V_t^{-1}}\\
    &\leq \gamma_{T, T}(\delta/4) \sqrt{2Td\log\bigg(1 + \frac{T L ^2}{d\lambda}\bigg)}\quad\text{(Lemma \ref{lemma:elliptical_potential_revisited})}.\\
\end{align*}


\begin{align*}
    \sum_{t=1}^T R_{t, T}^{\text{TS, c}}\ind_{E_t} &\leq \sum_{t=1}^T \lvert R_{t, T}^{\text{TS, c}} \rvert\ind_{E_t} \\
    &\leq \gamma_{T, T}(\delta/4)\sum_{t=1}^T \lVert X_t \rVert_{V_t^{-1}}\\
    &\leq \gamma_{T, T}(\delta/4) \sqrt{2Td\log\bigg(1 + \frac{T L ^2}{d\lambda}\bigg)}\quad\text{(Lemma \ref{lemma:elliptical_potential_revisited})}.\\
\end{align*}


\paragraph{Bounding $R_T^{\psi}$}\ \\

Similarly, we have

\begin{align*}
    \lvert R_{t, T}^{\psi}\rvert \ind_{E_t} &= \lvert X_t^\top (\wh{\theta}_t - \theta^*)\rvert \ind_{E_t}\\
    &= \lvert X_t^\top V_t^{-\frac{1}{2}} V_t^{\frac{1}{2}}(\wh{\theta}_t - \theta^*)\rvert \ind_{E_t}\\
    &\leq \lVert X_t \rVert_{V_t^{-1}} \lVert \wh{\theta}_t - \theta^*\rVert_{V_t} \ind_{E_t}\quad \text{(Cauchy-Schwarz)}\\
    &\leq \alpha_{t}(\delta/4)\lVert X_t \rVert_{V_t^{-1}} \quad \text{(concentration of $\wh{\theta}$)}\\
    &\leq \alpha_{t}(\delta/4)\lVert X_t \rVert_{V_t^{-1}}.\\
\end{align*}

Another application of lemma \ref{lemma:elliptical_potential_revisited} yields:
\[\sum_{t=1}^T R_{t, T}^{\psi}\ind_{E_t} \leq \alpha_{T}(\delta/4) \sqrt{2Td\log\bigg(1 + \frac{T L ^2}{d\lambda}\bigg)} \]

\end{proof}

==> convex_risk_ts_proofs.tex <==
\section{Proofs of lemmas for $\psi$-TS}\label{appendix:proof_ts}

\begin{proof}[Proof of Proposition \ref{prop:concentration_subgaussian_vectors}]\ \\

Let's fix $t\in\N$ and some $\epsilon>0$ to be determined later. We have

\[ \bP\left( \lVert \xi_t \rVert_2 \leq \epsilon \sqrt{d}\right)  \geq \bP\left( \forall j\in\{1, \dots, d\}, \lvert \xi_{j, t} \rvert \leq \epsilon\right)  \geq 1 - \sum_{j=1}^d \bP\left( \lvert \xi_{j, t} \rvert > \epsilon\right) \]
where the last inequality follows from the union bound on the $d$ coordinates. Each $\xi_{j, t}$ is a centred $\sigma_{\xi}$-sub-Gaussian (take $u=e_j$ the $j$-th vector of the canonical basis of $\R^d$ in the definition of sub-Gaussian vectors), therefore 
\[\forall j\in\{1, \dots, d\}, \bP\left( \lvert \xi_{j, t} \rvert > \epsilon\right) \leq  2 e^{-\frac{\epsilon^2}{2\sigma^2_{\xi}}}\]
which leads to 
\[ \bP\left( \lVert \xi_t \rVert_2 \leq \epsilon \sqrt{d}\right) \geq 1 - 2d e^{-\frac{\epsilon^2}{2\sigma^2_{\xi}}}.\]

The choice of $\epsilon = \sigma_{\xi} \sqrt{2d\log\frac{2d}{\delta}}$ yields the desired bound.

For the uniform bound, simply apply a union bound over $t=1, \dots, T$: 

\begin{align*}
    \bP\left( \forall t\leq T, \lVert \xi_t\rVert_2\leq \sigma_{\xi}\sqrt{2d\log\frac{2dT}{\delta}}\right)  &= 1 - \bP\left( \bigcup_{t=1}^T \Big\{ \lVert \xi_t\rVert_2 > \sigma_{\xi}\sqrt{2d\log\frac{2dT}{\delta}} \Big\} \right) \\
    &\geq 1 - \sum_{t=1}^T \bP\left( \lVert \xi_t\rVert_2 > \sigma_{\xi}\sqrt{2d\log\frac{2dT}{\delta}} \right) \\
    &\geq 1 - \sum_{t=1}^T \frac{\delta}{T} \\
    &= 1 - \delta.\\
\end{align*}
\end{proof}


==> erratum.tex <==
{\color{blue}
\section*{ERRATUM}

While finishing the supplementary material, we noticed two small typos in \textbf{Theorem~\ref{thm:regret_ucb-ogd}}. These are minor changes that do \textbf{not} significantly change the result. For readability, we have fixed them in the current document, and report below the exact changes.

\begin{itemize}
	\item {\color{red} $h=\lceil \frac{2\epsilon_h}{\rho_{\cX}L^2} + \frac{4}{\rho_{\cX}^2L^2}\log\frac{2}{\delta}\rceil$} should be replaced with $h=\lceil \frac{2\epsilon_h}{\rho_{\cX}L^2} + \frac{8}{\rho_{\cX}^2}\log\frac{2}{\delta}\rceil$.
	\item The constant $C$ in the definition of $c^{\text{OGD}, \delta}_{t, T}$ is not the same as the constant in the upper bound on $\cR_T$; we have renamed the former $C'$.
\end{itemize}

}

==> templates/articles/tikzhighlight.tex <==


\usetikzlibrary{calc}

\definecolor{bleugris}{RGB}{15,107,154}
\definecolor{myred}{RGB}{200,107,54}

\definecolor{darkyellow}{RGB}{233,165,0}  % orange S
\definecolor{lightgray}{rgb}{0.9,0.9,0.9}
\definecolor{darkgray}{rgb}{0.5,0.5,0.5}
\definecolor{rouge1}{RGB}{226,0,38}  % red P
\definecolor{rouge2}{RGB}{230,68,57}  % red S
\definecolor{orange2}{RGB}{236,117,40}  % orange S
\definecolor{orange1}{RGB}{243,154,38}  % orange P
\definecolor{jaune}{RGB}{254,205,27}  % jaune P
\definecolor{jaune2}{RGB}{226,181,23}  % jaune P
\definecolor{blanc}{RGB}{255,255,255} % blanc P
\definecolor{gris}{RGB}{91,94,111} % gris S
\definecolor{gris1}{RGB}{130,130,130} % gris S
\definecolor{bleu1}{RGB}{38,109,131} % bleu S
\definecolor{bleu2}{RGB}{28,50,114} % bleu S
\definecolor{blue3}{RGB}{0,0.2,0.9}
\definecolor{blue4}{RGB}{100,149,237}
\definecolor{vert1}{RGB}{133,146,66} % vert S
\definecolor{vert3}{RGB}{20,200,66} % vert S
\definecolor{vert2}{RGB}{157,193,7} % vert S
\definecolor{vert4}{RGB}{20,200,20} % vert S
\definecolor{indigo}{RGB}{75,0,130}
\definecolor{plum}{RGB}{221,160,221}
\definecolor{taupe}{RGB}{134,113,127} % taupe S
\definecolor{purple}{RGB}{200,100,200} % taupe S
\definecolor{brown}{RGB}{121,77,20} % taupe S


\tikzset{
	invisible/.style={opacity=0,text opacity=0},
	visible on/.style={alt=#1{}{invisible}},
	alt/.code args={<#1>#2#3}{%
		\alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}} 
	},
	background fill/.style={fill=#1},
	background fill/.default={white},
	fill on/.style={alt=#1{}{background fill}},
	background draw/.style={draw=#1},
	background draw/.default={white},
	draw on/.style={alt=#1{}{background draw}},
	background filldraw/.style args={#1 filled by #2}{draw=#1, fill=#2},
	background filldraw/.default=white filled by white,
	filldraw on/.style={alt=#1{}{background filldraw}},
}

\tikzset{bluehighlighting/.style={
		append after command={
			\pgfextra{
				\path[rounded corners,
				background filldraw=orange filled by bleugris!99, % border+filling
				%filldraw on=<#1>, % overlay specification
				overlay] ($(\tikzlastnode.south west)+(-0.05,-0.08)$) % to have some offset
				rectangle ($(\tikzlastnode.north east)+(0.05,0.1)$);
			}   
		}
	}
}

\tikzset{redhighlighting/.style={
		append after command={
			\pgfextra{
				\path[rounded corners,
				background filldraw=orange filled by rouge1!99, % border+filling
				%filldraw on=<#1>, % overlay specification
				overlay] ($(\tikzlastnode.south west)+(-0.05,-0.08)$) % to have some offset
				rectangle ($(\tikzlastnode.north east)+(0.05,0.1)$);
			}   
		}
	}
}

\tikzset{orangehighlighting/.style={
		append after command={
			\pgfextra{
				\path[rounded corners,
				background filldraw=orange filled by orange1!99, % border+filling
				%filldraw on=<#1>, % overlay specification
				overlay] ($(\tikzlastnode.south west)+(-0.05,-0.08)$) % to have some offset
				rectangle ($(\tikzlastnode.north east)+(0.05,0.1)$);
			}   
		}
	}
}

\tikzset{greenhighlighting/.style={
		append after command={
			\pgfextra{
				\path[rounded corners,
				background filldraw=orange filled by vert4!99, % border+filling
				%filldraw on=<#1>, % overlay specification
				overlay] ($(\tikzlastnode.south west)+(-0.05,-0.08)$) % to have some offset
				rectangle ($(\tikzlastnode.north east)+(0.05,0.1)$);
			}   
		}
	}
}

\tikzset{purplehighlighting/.style={
		append after command={
			\pgfextra{
				\path[rounded corners,
				background filldraw=orange filled by purple!99, % border+filling
				%filldraw on=<#1>, % overlay specification
				overlay] ($(\tikzlastnode.south west)+(-0.05,-0.08)$) % to have some offset
				rectangle ($(\tikzlastnode.north east)+(0.05,0.1)$);
			}   
		}
	}
}


\tikzset{yellowhighlighting/.style={
		append after command={
			\pgfextra{
				\path[rounded corners,
				background filldraw=orange filled by jaune2!99, % border+filling
				%filldraw on=<#1>, % overlay specification
				overlay] ($(\tikzlastnode.south west)+(-0.05,-0.08)$) % to have some offset
				rectangle ($(\tikzlastnode.north east)+(0.05,0.1)$);
			}   
		}
	}
}


\tikzset{brownhighlighting/.style={
		append after command={
			\pgfextra{
				\path[rounded corners,
				background filldraw=orange filled by brown!99, % border+filling
				%filldraw on=<#1>, % overlay specification
				overlay] ($(\tikzlastnode.south west)+(-0.05,-0.08)$) % to have some offset
				rectangle ($(\tikzlastnode.north east)+(0.05,0.1)$);
			}   
		}
	}
}


\tikzset{cyanhighlighting/.style={
		append after command={
			\pgfextra{
				\path[rounded corners,
				background filldraw=orange filled by blue4!99, % border+filling
				%filldraw on=<#1>, % overlay specification
				overlay] ($(\tikzlastnode.south west)+(-0.05,-0.08)$) % to have some offset
				rectangle ($(\tikzlastnode.north east)+(0.05,0.1)$);
			}   
		}
	}
}



\tikzset{silverhighlighting/.style={
		append after command={
			\pgfextra{
				\path[rounded corners,
				background filldraw=orange filled by gris1!99, % border+filling
				%filldraw on=<#1>, % overlay specification
				overlay] ($(\tikzlastnode.south west)+(-0.05,-0.08)$) % to have some offset
				rectangle ($(\tikzlastnode.north east)+(0.05,0.1)$);
			}   
		}
	}
}



\tikzset{darkhighlighting/.style={
		append after command={
			\pgfextra{
				\path[rounded corners,
				background filldraw=orange filled by black!99, % border+filling
				%filldraw on=<#1>, % overlay specification
				overlay] ($(\tikzlastnode.south west)+(-0.05,-0.08)$) % to have some offset
				rectangle ($(\tikzlastnode.north east)+(0.05,0.1)$);
			}   
		}
	}
}

\newcommand{\hlb}[1]{%
	\tikz[baseline=(A.base)] 
	\node[bluehighlighting,inner sep=0pt] (A) {\bf{\textcolor{white}{#1}}};%
}
\newcommand{\hlr}[1]{%
	\tikz[baseline=(A.base)] 
	\node[redhighlighting,inner sep=0pt] (A) {\bf{\textcolor{white}{#1}}};%
}
\newcommand{\hlo}[1]{%
\tikz[baseline=(A.base)] 
\node[orangehighlighting,inner sep=0pt] (A) {\bf{\textcolor{white}{#1}}};%
}
\newcommand{\hlg}[1]{%
	\tikz[baseline=(A.base)] 
	\node[greenhighlighting,inner sep=0pt] (A) {\bf{\textcolor{white}{#1}}};%
}
\newcommand{\hlp}[1]{%
	\tikz[baseline=(A.base)] 
	\node[purplehighlighting,inner sep=0pt] (A) {\bf{\textcolor{white}{#1}}};%
}
\newcommand{\hly}[1]{%
\tikz[baseline=(A.base)] 
\node[yellowhighlighting,inner sep=0pt] (A) {\bf{\textcolor{white}{#1}}};%
}
\newcommand{\hlm}[1]{%
\tikz[baseline=(A.base)] 
\node[brownhighlighting,inner sep=0pt] (A) {\bf{\textcolor{white}{#1}}};%
}
\newcommand{\hlc}[1]{%
\tikz[baseline=(A.base)] 
\node[cyanhighlighting,inner sep=0pt] (A) {\bf{\textcolor{white}{#1}}};%
}

\newcommand{\hls}[1]{%
	\tikz[baseline=(A.base)] 
	\node[silverhighlighting,inner sep=0pt] (A) {\bf{\textcolor{white}{#1}}};%
}

\newcommand{\hlk}[1]{%
	\tikz[baseline=(A.base)] 
	\node[darkhighlighting,inner sep=0pt] (A) {\bf{\textcolor{white}{#1}}};%
}

==> templates/style/beamer.tex <==

% Layout
\usetheme{default}
\geometry{paperwidth=140mm,paperheight=105mm}
\useoutertheme{infolines}
\usepackage{layout}
\usepackage{fancybox}
\usepackage[absolute,showboxes,overlay]{textpos}

\TPshowboxesfalse
\textblockorigin{0mm}{0mm}


% Colors
\usepackage{colortbl}
\usepackage{xcolor,colortbl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\xdefinecolor{lgreen}{rgb}{0.0,0.6,0.0}
\xdefinecolor{ugreen}{rgb}{0.9,1.,0.9}
\xdefinecolor{lorange}{rgb}{0.8,0.3,0.0}
\xdefinecolor{uorange}{rgb}{0.9,0.85,0.8}
\xdefinecolor{lyellow}{rgb}{0.8,0.7,0.0}
\xdefinecolor{uyellow}{rgb}{1.,0.9,0.8}
\xdefinecolor{lblue}{rgb}{0.2,0.2,0.8}
\xdefinecolor{lred}{rgb}{0.8,0.,0.}
\xdefinecolor{lcyan}{rgb}{0.3,0.3,1}
\xdefinecolor{myorange}{rgb}{1.,0.15,0.}
\xdefinecolor{mypink}{rgb}{1.,0.0,0.5}
\xdefinecolor{mygreen}{rgb}{0.,0.6,0.1}
\definecolor{darkyellow}{RGB}{233,165,0}  % orange S
\definecolor{lightgray}{rgb}{0.9,0.9,0.9}
\definecolor{darkgray}{rgb}{0.5,0.5,0.5}
\definecolor{rouge1}{RGB}{226,0,38}  % red P
\definecolor{rouge2}{RGB}{230,68,57}  % red S
\definecolor{orange2}{RGB}{236,117,40}  % orange S
\definecolor{orange1}{RGB}{243,154,38}  % orange P
\definecolor{jaune}{RGB}{254,205,27}  % jaune P
\definecolor{blanc}{RGB}{255,255,255} % blanc P
\definecolor{gris}{RGB}{91,94,111} % gris S
\definecolor{bleu1}{RGB}{38,109,131} % bleu S
\definecolor{bleu2}{RGB}{28,50,114} % bleu S
\definecolor{blue3}{RGB}{0,0.2,0.9}
\definecolor{blue4}{RGB}{100,149,237}
\definecolor{vert1}{RGB}{133,146,66} % vert S
\definecolor{vert3}{RGB}{20,200,66} % vert S
\definecolor{vert2}{RGB}{157,193,7} % vert S
\definecolor{vert4}{RGB}{20,200,20} % vert S
\definecolor{indigo}{RGB}{75,0,130}
\definecolor{plum}{RGB}{221,160,221}
\definecolor{taupe}{RGB}{134,113,127} % taupe S


% Highlights for slides
\newcommand{\red}{\color{lred}}
\newcommand{\black}{\color{black}}
\newcommand{\orange}{\color{myorange}}
\newcommand{\hl}[1]{{\color{mypink} #1}}
\newcommand{\gl}[1]{{\color{gray!70!black} #1}}
\newcommand{\HL}[1]{{\color{red!100!black} #1}}
\newcommand{\eg}[1]{{\color{mygreen} #1}}
\newcommand{\mycite}[1]{{\color{blue!80!black}#1}}
\newcommand{\rcol}[1]{\textcolor{red}{\textit{#1}}}
\newcommand{\eqrcol}[1]{\textcolor{red}{#1}}
\newcommand{\pcol}[1]{\textcolor{plum}{\textit{#1}}}
\newcommand{\eqpcol}[1]{\textcolor{plum}{#1}}
\newcommand{\gcol}[1]{\textcolor{vert3}{\textit{#1}}}
\newcommand{\eqgcol}[1]{\textcolor{vert3}{#1}}
\newcommand{\bcol}[1]{\textcolor{blue}{\textit{#1}}}
\newcommand{\eqbcol}[1]{\textcolor{blue}{#1}}
\newcommand{\ycol}[1]{\textcolor{darkyellow}{\textit{#1}}}
\newcommand{\eqycol}[1]{\textcolor{darkyellow}{#1}}
\newcommand{\rcolb}[1]{\textcolor{red}{\textit{\textbf{#1}}}}
\newcommand{\gcolb}[1]{\textcolor{vert3}{\textit{\textbf{#1}}}}
\newcommand{\bcolb}[1]{\textcolor{blue}{\textit{\textbf{#1}}}}
\newcommand{\ycolb}[1]{\textcolor{darkyellow}{\textit{\textbf{#1}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\renewcommand{\sfdefault}{lmss}
\sffamily

% Custom beamer blocks
\newenvironment<>{orangeblock}[1]{%
	\setbeamercolor{block title}{fg=white,bg=orange}%
	\setbeamercolor*{block body}{fg=black, bg= orange!5}
	\begin{block} #2{#1}}{ \end{block}}

\newcommand{\shadedtitle}[3]{
	\setlength{\fboxsep}{0pt}%
	\setlength{\fboxrule}{1pt}%
	%	\begin{textblock}{12.6}(0.,0.75)
	%		\begin{tikzpicture}
	%		\node[top color=black,bottom color=white] 
	%		{
	%			\begin{minipage}[t][0cm][b]{12.6cm}
	%			{.}
	%			\end{minipage}
	%		};
	%		\end{tikzpicture}
	%	\end{textblock}
	\begin{textblock}{12.6}(0,0)
		\begin{tikzpicture}
		%		\node[left color=#2, right color=#3] 
		\node[inner color=#3,outer color=#2] 
		{
			\begin{minipage}[t][7pt][t]{\paperwidth}
			\begin{center}
			{\Large #1}
			\end{center}
			\end{minipage}
		};
		\end{tikzpicture}	
		%			\begin{tikzpicture}
		%		\node[left color=#2, right color=#3] at (0,0)
		%		{
		%			\phantom{\hspace{0.5\paperwidth}}
		%		};
		%		\node[left color=#3, right color=#2] at (0.5\paperwidth,0)
		%		{
		%			\phantom{\hspace{0.5\paperwidth}}
		%		};	
		%		\node at (0,0)
		%		{
		%%				\begin{minipage}[t][7pt][t]{\paperwidth}
		%%					\begin{center}
		%					#1
		%%					\end{center}
		%%				\end{minipage}
		%		};
		%		\end{tikzpicture}
		
	\end{textblock}
}


% Sections and TOC
\setbeamertemplate{section in toc}
{\centering \textsc{\inserttocsection} \\}

\setbeamertemplate{subsection in toc}
{\centering \inserttocsubsection \\}

\def\Vhrulefill{\leavevmode\leaders\hrule height 0.7ex depth \dimexpr0.4pt-0.7ex\hfill\kern0pt}
\def\Vhrule{\leavevmode\leaders\hrule height 0.7ex depth \dimexpr0.4pt-0.7ex\hrule\kern0pt}


\makeatletter
\def\beamer@tocaction@bold#1{\Vhrulefill\\ \vspace{-2.5ex}\centering  \textbf{\LARGE	\colorbox{white}{~~\inserttocsubsection~~}} \\}
%\def\beamer@tocaction@bold#1{\only<.(1)>{\usebeamertemplate**{#1}}}
%\define@key{beamertoc}{subsectionsonly}[]{\beamer@toc@subsectionstyle{show/only}\beamer@toc@subsubsectionstyle{show/shaded/hide}}
\makeatother


\AtBeginSection{
	\begin{frame}[noframenumbering]\frametitle{Table of contents}
		\Large%
		%	\tableofcontents[sectionstyle=show/shaded%
		%	,subsectionstyle=shaded/shaded/hide]
		\tableofcontents[sectionstyle=show/shaded%
		,subsectionstyle=hide/hide/hide]
	\end{frame}
}

\AtBeginSubsection{ 
	\begin{frame}[noframenumbering,c]\frametitle{Table of contents}
		\Large%
		\tableofcontents[sectionstyle=show/shaded%
		,subsectionstyle=bold/shaded/hide]
	\end{frame}
}





% Change margins for slides
\newenvironment{changemargin}[2]{% 
	\begin{list}{}{% 
			\setlength{\topsep}{0pt}% 
			\setlength{\leftmargin}{#1}% 
			\setlength{\rightmargin}{#2}% 
			\setlength{\listparindent}{\parindent}% 
			\setlength{\itemindent}{\parindent}% 
			\setlength{\parsep}{\parskip}% 
		}% 
		\item[]}{\end{list}} 
